Efficient Network Reliability Computation in Uncertain Graphs

Network reliability is an important metric to evaluate the connectivity among given vertices in uncertain graphs. Since the network reliability problem is known as #P-complete, existing studies have used approximation techniques. In this paper, we propose a new sampling-based approach that efficiently and accurately approximates network reliability. Our approach improves efficiency by reducing the number of samples based on stratified sampling. We theoretically guarantee that our approach improves the accuracy of approximation by using lower and upper bounds of network reliability, even though it reduces the number of samples. To efficiently compute the bounds, we develop an extended BDD, called S2BDD. During constructing the S2BDD, our approach employs dynamic programming for efficiently sampling possible graphs. Our experiment with real datasets demonstrates that our approach is up to 51.2 times faster than the existing sampling-based approach with higher accuracy.

==> algorithms/checkterminal.tex <==
\begin{algorithm}[!t]
{\scriptsize
	\caption{Updating nodes in the S$^2$BDD}	\label{alg:check}
		\DontPrintSemicolon
		  \SetKwFunction{update}{update}
            	{\bf procedure} \update{$n$, $\mathbb{F}'$, $\mathbb{F}$, $state$, $\mathcal{G}$, $e_l$}\\
            	$n' \leftarrow n$;\\
            	\For{$f \in \mathbb{F}$}{
            		            	\If{$f \in \mathbb{F}'$}{
            			            	$c_{n,f} \leftarrow c_{n',f}$; $d_{n,f} \leftarrow d_{n',f}$;  $t_{n,f} \leftarrow t_{n',f}$;\\
            		            	}
            	    		        \Else{
	            	    		        $c_{n,f} \leftarrow f$; $d_{n,f} \leftarrow$ degree of $f$ in $\mathcal{G}$; \\
	            	    		        {\bf if} $f \in \mathbb{T}$ {\bf then} $t_{n,f} \leftarrow$ 1 {\bf else} $t_{n,f} \leftarrow$ 0;\\
            	        		    }
            	            	}
            	            	\If{$\mathit{state}$ is existent}{
	            	            	$p_n \leftarrow p_n \cdot p(e_l)$;\\
            			        	update $c_{n,f}, d_{n,f}, t_{n,f}$ for $\forall f \in \mathbb{F}_{n}$;\\
            			        	%$c_{min} \leftarrow min(n.comp[u], n.comp[w])$;\\
            			        	%$c_{max} \leftarrow max(n.comp[u], n.comp[w])$;\\
            			        	%$deg \leftarrow n.deg[c_{max}]$;\\
            			        	%\If{$c_{min} \neq c_{max}$}{
            				       % 	\For{$v \in F_c.size$}{
            					     %   	\If{$n.comp[v] = c_{max}$}{
            					      %  	$n.comp[v] = c_{min}$;}
            				        %	}
            				        %	\For{$v \in F_c.size$}{
            					      %  	\If{$n.comp[v] = c_{min}$}{
            					      %  	$n.deg[v] = deg$;}
            				        %	}
            			        	%}
            			        	\If{for $\exists f \in \mathbb{F},  t_{n,f}$ is $k$}{{\bf return} 1-sink;\tcc*[r]{Lemma 1}}
            			        	\If{$v \in \mathbb{F}'$  {\bf and} $v' \in \mathbb{F}' \cup \mathbb{F}$ {\bf and} $t_{n',v} = k-1$ {\bf and} $v' \in \mathbb{T}$}{{\bf return} 1-sink;\tcc*[r]{Lemma 2}}
            			        	\If{$v ,v' \in \mathbb{F}'$  {\bf and} $t_{n',v} + t_{n',v'} = k$ {\bf and} $c_{n',v} \neq c_{n',v'}$}{{\bf return} 1-sink;\tcc*[r]{Lemma 3}}
            			        	\If{$v ,v' \in \mathbb{F}' \backslash \mathbb{F}$ {\bf and} $(t_{n',v}>0$ {\bf or} $t_{n',v'}>0)$}{{\bf return} 0-sink;\tcc*[r]{Lemma 6}}
            	            	}
            	            	\If{$state$ is non-existent}{
	            	            	$p_n \leftarrow p_n \cdot (1-p(e_l))$;\\
	            	            	update $d_{n,f}$ for $\forall f \in \mathbb{F}$;\\
	            	            	\If{$v \in \mathbb{F}'$ {\bf and} $t_{n',v}>0$ {\bf and} $d_{n',v}=1$}{{\bf return} 0-sink;\tcc*[r]{Lemma 4}}
	            	            	\If{$v  \in \mathbb{F}' \cup \mathbb{F}$ {\bf and} $v \in \mathbb{T}$ }{{\bf return} 0-sink;\tcc*[r]{Lemma 5}}
									\If{$v ,v' \in \mathbb{F}' \backslash \mathbb{F}$ {\bf and} $(t_{n',v}>0$ {\bf or} $t_{n',v'}>0)$}{{\bf return} 0-sink;\tcc*[r]{Lemma 6}}
            	            	}
              {\bf return} $n$;\\    
              {\bf end procedure}
              }
\end{algorithm}

